Spectral energy distribution similarity of the local galaxies and the 3.6um selected galaxies from the Spitzer Extended Deep Survey

The Spitzer Extended Deep Survey (SEDS) as a deep and wide mid-infrared (MIR) survey project provides a sample of 500000+ sources spreading 1.46 square degree and a depth of 26 AB mag (3$\sigma$). Combining with the previous available data, we build a PSF-matched multi-wavelength photometry catalog from u band to 8$\mu$m. We fit the SEDS galaxies spectral energy distributions by the local galaxy templates. The results show that the SEDS galaxy can be fitted well, indicating the high redshift galaxy ($z \sim 1$) shares the same templates with the local galaxies. This study would facilitate the further study of the galaxy luminosity and high redshift mass function.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

